Computing in the Era of Large Generative Models: From Cloud-Native to AI-Native

In this paper, we investigate the intersection of large generative AI models and cloud-native computing architectures. Recent large models such as ChatGPT, while revolutionary in their capabilities, face challenges like escalating costs and demand for high-end GPUs. Drawing analogies between large-model-as-a-service (LMaaS) and cloud database-as-a-service (DBaaS), we describe an AI-native computing paradigm that harnesses the power of both cloud-native technologies (e.g., multi-tenancy and serverless computing) and advanced machine learning runtime (e.g., batched LoRA inference). These joint efforts aim to optimize costs-of-goods-sold (COGS) and improve resource accessibility. The journey of merging these two domains is just at the beginning and we hope to stimulate future research and development in this area.

==> Makefile <==
###############################################################################
# Project Configuration

TARGET				:= $(shell basename $(PWD)).pdf
MAIN					:= main

#####

TARGET_BASE 	:= $(basename $(TARGET))

################################################################################
# Command Configuration

PDFLATEX			:= pdflatex
BIBTEX				:= bibtex
EPS_TO_PDF		:= epstopdf
OBJ_TO_EPS		:= tgif -print -eps -color -stdout
GNUPLOT				:= gnuplot
SPELLCHECK		:= aspell -c -t --lang=en --personal=$(shell pwd)/ignore.aspell 

################################################################################
# Gathering Information

TEX_MAIN := $(MAIN).tex

TEX_ALL := $(shell search=$(TEX_MAIN); all=; \
				while [ -n "$$search" ] ; do \
					all="$$all $$search"; \
					search=`egrep '^[^%]*\\\\(input|include)' $$search | \
						sed -En 's/.*(input|include)(\[[^\]]\])?\{(.+)\}.*/\3.tex/p'`; \
				done; \
				echo "$$all")

GFX_ALL := $(shell for t in $(TEX_ALL); do \
				cat $$t | \
				egrep '^[^%]*\\includegraphics' | \
				sed -En 's/.*includegraphics(\[.+\])?\{([^\{}]*)\}.*/\2/p'; \
				done)

GFX_FILES := $(shell for g in $(GFX_ALL); do \
					ls $$g.* | \
					egrep "(\.obj|\.eps)$$" | \
					sed -E 's/\.[^ ]+/\.pdf/g'; \
					done)

GNUPLOT_FILES := $(shell for g in $(GFX_ALL); do \
							test -e $$g.p && \
							test ! -e $$g.eps -a ! -e $$g.obj && \
							echo $$g.pdf; \
							done)

BIB_FILES := $(shell cat $(TEX_MAIN) | \
					egrep '^[^%]*\\bibliography\{' | \
					sed -E -e 's/.*\{([^\{]+)\}.*/\1/g' \
						-e 's/([^,\{\}]+)/\1.bib/g' \
						-e 's/,/ /g')	

################################################################################
# Command Rules

all: $(TARGET)

$(TARGET): $(TEX_ALL) $(GFX_FILES) $(GNUPLOT_FILES) $(BIB_FILES)
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	-$(BIBTEX) $(MAIN)
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	mv $(MAIN).pdf $@

debug:
	@echo "TEX_MAIN = $(TEX_MAIN)"
	@echo "TEX_ALL = $(TEX_ALL)"
	@echo "GFX_ALL = $(GFX_ALL)"
	@echo "GFX_FILES = $(GFX_FILES)"
	@echo "GNUPLOT_FILES = $(GNUPLOT_FILES)"
	@echo "BIB_FILES = $(BIB_FILES)"

clean:
	rm -f $(TARGET) $(TARGET_BASE)-gray.pdf $(TARGET_BASE)-final.pdf \
		*~ *.bbl *.blg *.log *.aux *.toc *.lof *.lot $(MAIN).out $(GFX_FILES) $(GNUPLOT_FILES)

grayscale: $(TARGET_BASE)-gray.pdf

$(TARGET_BASE)-gray.pdf: $(TARGET)
	gs -sOutputFile=$@ -sDEVICE=pdfwrite -sColorConversionStrategy=Gray \
		-dProcessColorModel=/DeviceGray -dNOPAUSE \
		-dBATCH -dAutoRotatePages=/None $(TARGET)

finalized: $(TARGET_BASE)-final.pdf

$(TARGET_BASE)-final.pdf: $(TEX_ALL) $(GFX_FILES) $(GNUPLOT_FILES) $(BIB_FILES)
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	-$(BIBTEX) $(MAIN)
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	mv $(MAIN).pdf $@

spellcheck: $(TEX_ALL:.tex=.spell)


################################################################################
# File -> File Rules

%.pdf: %.eps
	$(EPS_TO_PDF) $<

%.pdf: %.obj
	$(OBJ_TO_EPS) $< | \
	$(EPS_TO_PDF) -f -o=$@

%.pdf: %.p
	$(GNUPLOT) $< | \
	$(EPS_TO_PDF) -f -o=$@

%.spell: %.tex
	$(SPELLCHECK) $<



==> abstract.tex <==
\section*{Abstract}


==> cmds.tex <==
\renewcommand{\ttdefault}{pxtt}

% \newcommand{\URL}{\url}
\newcommand{\cc}[1]{\mbox{\smaller[0.5]\texttt{#1}}}

%\clubpenalty=10000
%\widowpenalty=10000

%\linespread{1.2}

\fvset{fontsize=\scriptsize,xleftmargin=8pt,numbers=left,numbersep=5pt}

\input{code/fmt}
\newcommand{\figrule}{\hrule width \hsize height .33pt}
\newcommand{\coderule}{\vspace{-0.4em}\figrule}

\setlength{\abovedisplayskip}{0pt}
\setlength{\abovedisplayshortskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength{\belowdisplayshortskip}{0pt}
\setlength{\jot}{0pt}

\def\Snospace~{\S{}}
%\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{\Snospace}
\def\subsectionautorefname{\Snospace}
\def\subsubsectionautorefname{\Snospace}
\def\chapterautorefname{\Snospace}
\def\equationautorefname{Eqn.}

%\renewcommand{\figurename}{Fig.}
%\def\figureautorefname{\figurename}
% \newcommand{\subfigureautorefname}{\figureautorefname}

\numberwithin{equation}{section}
\newcommand{\yes}{Y}
\newcommand{\no}{}

% sema
\newcommand{\shl}{\ \cc{<}\cc{<}\ }
\newcommand{\shr}{\ \cc{>}\cc{>}\ }

\if 0
\renewcommand{\topfraction}{0.9}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.9}
\setcounter{topnumber}{10}
\setcounter{bottomnumber}{10}
\setcounter{totalnumber}{10}
\setcounter{dbltopnumber}{10}
\fi

\newif\ifdraft\drafttrue
\newif\ifnotes\notestrue
\ifdraft\else\notesfalse\fi

% per-author notes:
% ref. http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand{\BH}[1]{\textcolor{Green}{BH: #1}}
\newcommand{\CV}[1]{\textcolor{Orange}{BH: #1}}
\newcommand{\QZ}[1]{\textcolor{Red}{QZ: #1}}
\newcommand{\AJ}[1]{\textcolor{green}{AJ: #1}}

\newcommand{\TODO}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\COMMENT}[1]{\textcolor{blue}{(#1)}}

%% Ensure ligatures (e.g., ``fine official flag'') can be copy/pasted from PDF.
\input{glyphtounicode}
\pdfgentounicode=1

\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

% include macros
\newcommand{\includepdf}[1]{
  \includegraphics[width=\columnwidth]{#1}
}

\newcommand{\includeplot}[1]{
  \resizebox{\columnwidth}{!}{\input{#1}}
}

%% NOTE.
%%  to use circled number in caption, use
%%   (e.g., \protect\C{1})
%%

\newcommand*\BC[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,fill=black,inner sep=0.2pt](C) {\textcolor{white}{#1}};
\end{tikzpicture}}

\newcommand{\PP}[1]{
\vspace{2px}
\noindent{\bf\textsc{#1}.}\xspace
}

\newcommand{\PPS}[1]{
\noindent{\bf\textsc{#1}}
}
% % Squished Lists
\newcommand{\squishitemize}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{0pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.95em}
     \setlength{\labelwidth}{1.5em}
     \setlength{\labelsep}{0.5em} } }

\newcounter{Lcount}
\newcommand{\squishlist}{
    \begin{list}{\arabic{Lcount}. }
   { \usecounter{Lcount}
        \setlength{\itemsep}{0pt}
        \setlength{\parsep}{3pt}
        \setlength{\topsep}{0pt}
        \setlength{\partopsep}{0pt}
        \setlength{\leftmargin}{2em}
        \setlength{\labelwidth}{1.5em}
        \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{\end{list}}

\usepackage{xstring}

\newcommand{\eg}{\textit{e}.\textit{g}.,\xspace}
\newcommand{\ie}{\textit{i}.\textit{e}.,\xspace}
\newcommand{\etc}{\textit{e}.\textit{t}.\textit{c}.}

% Systems
\newcommand{\opt}{\textsc{query planner}\xspace}
\newcommand{\proc}{\textsc{query processor}\xspace}

\renewcommand{\sys}{\textsc{Zeus}\xspace}
\newcommand{\rl}{\textsc{RL}\xspace}
\newcommand{\udf}{\textsc{UDF}\xspace}

\newcommand{\qa}{\texttt{Q1}\xspace}
\newcommand{\qb}{\texttt{Q2}\xspace}
\newcommand{\qc}{\texttt{Q3}\xspace}
\newcommand{\qd}{\texttt{Q4}\xspace}
\newcommand{\qe}{\texttt{Q5}\xspace}
\newcommand{\qf}{\texttt{Q6}\xspace}

% Models

\newcommand{\rthreed}{\texttt{\textsc{R3D}}\xspace}


\newcommand{\dcircle}[1]{\ding{\numexpr181 + #1}}


% Custom
\newcommand{\rpm}{\sbox0{$1$}\sbox2{$\scriptstyle\pm$}
  \raise\dimexpr(\ht0-\ht2)/2\relax\box2 }

==> code/code.tex <==
 

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/p1.java.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{p1} \PY{p}{(}\PY{k+kt}{int} \PY{n}{EMPNO}\PY{p}{,} \PY{n}{String} \PY{n}{ENAME}\PY{p}{,} \PY{k+kt}{int} \PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{DEPTNO} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{if}\PY{p}{(}\PY{n}{DEPTNO}\PY{o}{+}\PY{l+m+mi}{5}\PY{o}{\PYZgt{}} \PY{n}{EMPNO}\PY{p}{)}\PY{p}{\PYZob{}}
      \PY{k}{return} \PY{p}{(}\PY{n}{EMPNO}\PY{p}{,}\PY{n}{ENAME}\PY{p}{,}\PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}
\PY{n}{p2} \PY{p}{(}\PY{k+kt}{int} \PY{n}{EMPNO}\PY{p}{,} \PY{n}{String} \PY{n}{ENAME}\PY{p}{,} \PY{k+kt}{int} \PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZob{}}
  \PY{k}{if} \PY{p}{(}\PY{n}{DEPTNO} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)}\PY{p}{\PYZob{}}
    \PY{k}{if}\PY{p}{(}\PY{l+m+mi}{15}\PY{o}{\PYZgt{}} \PY{n}{EMPNO}\PY{p}{)}\PY{p}{\PYZob{}}
      \PY{k}{return} \PY{p}{(}\PY{n}{EMPNO}\PY{p}{,}\PY{n}{ENAME}\PY{p}{,}\PY{n}{DEPTNO}\PY{p}{)}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/q1.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{TABLE} \PY{n}{EMP}\PY{p}{(}\PY{n}{EMPNO} \PY{n+nb}{int}\PY{p}{,} \PY{n}{ENAME} \PY{n}{String}\PY{p}{,} \PY{n}{DEPTNO} \PY{n+nb}{int}\PY{p}{)}\PY{p}{;}
\PY{n}{Case1}\PY{p}{:}
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
     \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t} 
    \PY{k}{WHERE} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{t}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
     \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t1} 
    \PY{k}{WHERE} \PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{t1}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{;} 

\PY{n}{Case2}\PY{p}{:}
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{AS} \PY{n}{EMP} 
        \PY{k}{WHERE} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{o}{=} \PY{l+m+mi}{10} \PY{k}{AND} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{IS} \PY{k}{NOT} \PY{k}{NULL}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP0}\PY{p}{.}\PY{n}{EMPNO} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{AS} \PY{n}{EMP0} 
        \PY{k}{WHERE} \PY{n}{EMP0}\PY{p}{.}\PY{n}{EMPNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{;} 
\end{Verbatim}


==> code/q2.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{,} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{JOIN} \PY{n}{DEPT}
      \PY{k}{ON} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{=} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DEPTNO} \PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
      \PY{p}{(}\PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{,} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{LEFT} \PY{k}{OUTER} \PY{k}{JOIN} \PY{n}{DEPT}
         \PY{k}{ON} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{=} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{)}
    \PY{k}{WHERE} \PY{n}{DEPT}\PY{p}{.}\PY{n}{DNAME} \PY{k}{IS} \PY{k}{NOT} \PY{k}{NULL}
\end{Verbatim}


==> code/q3.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{k}{COUNT}\PY{p}{(}\PY{o}{*}\PY{p}{)} \PY{k}{FROM}
      \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
        \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t} 
      \PY{k}{WHERE} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{t}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{)}\PY{p}{;}

\PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{k}{COUNT}\PY{p}{(}\PY{o}{*}\PY{p}{)} \PY{k}{FROM}
      \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} 
        \PY{p}{(}\PY{k}{SELECT} \PY{o}{*} \PY{k}{FROM} \PY{n}{EMP} \PY{k}{WHERE} \PY{n}{DEPTNO} \PY{o}{=} \PY{l+m+mi}{10}\PY{p}{)} \PY{k}{AS} \PY{n}{t1} 
      \PY{k}{WHERE} \PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{t1}\PY{p}{.}\PY{n}{EMPNO}\PY{p}{)}\PY{p}{;} 
\end{Verbatim}


==> code/q4.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
  \PY{k}{TABLE} \PY{n}{EMP}\PY{p}{(}\PY{n}{EMPNO} \PY{n+nb}{int}\PY{p}{,} \PY{n}{ENAME} \PY{n}{String}\PY{p}{,} \PY{n}{DEPTNO} \PY{n+nb}{int}\PY{p}{,}\PY{n}{SAL} \PY{n+nb}{int}\PY{p}{)}\PY{p}{;}
  \PY{n}{q1}\PY{p}{:} \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{EMP}\PY{p}{.}\PY{n}{SAL}\PY{p}{)} 
      \PY{k}{FROM} \PY{n}{EMP} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}
  \PY{n}{q2}\PY{p}{:} \PY{k}{SELECT} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{t}\PY{p}{.}\PY{n}{sum1}\PY{p}{)} \PY{k}{FROM} \PY{p}{(}
   \PY{k}{SELECT} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{,} \PY{k}{SUM}\PY{p}{(}\PY{n}{EMP}\PY{p}{.}\PY{n}{SAL}\PY{p}{)} \PY{k}{as} \PY{n}{sum1}
    \PY{k}{FROM} \PY{n}{EMP} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{EMP}\PY{p}{.}\PY{n}{DEPTNO}\PY{p}{)} \PY{k}{AS} \PY{n}{t} \PY{k}{GROUP} \PY{k}{BY} \PY{n}{t}\PY{p}{.}\PY{n}{DEPTNO}
\end{Verbatim}


==> code/r1.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} 
\PY{n}{cond1}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{n}{v2} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{o}{!}\PY{n}{n2} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0}\PY{p}{)} \PY{p}{)} 
\PY{n}{cols1}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v0}\PY{p}{,}\PY{n}{n0}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v1}\PY{p}{,}\PY{n}{n1}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v2}\PY{p}{,}\PY{n}{n2}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign1}\PY{p}{:} \PY{k}{True}

\PY{n}{q2}\PY{p}{:} 
\PY{n}{cond2}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0} \PY{p}{)} 
\PY{n}{cols2}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v0}\PY{p}{,}\PY{n}{n0}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v1}\PY{p}{,}\PY{n}{n1}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{n}{v2}\PY{p}{,}\PY{n}{n2}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign2}\PY{p}{:} \PY{k}{True}
\end{Verbatim}


==> code/r2.sql.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n}{q1}\PY{p}{:} 
\PY{n}{cond1}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{n}{v2} \PY{o}{+} \PY{l+m+mi}{5} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{o}{!}\PY{n}{n2} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0}\PY{p}{)} \PY{p}{)} 
\PY{n}{cols1}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v3}\PY{p}{,}\PY{n}{isN3}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign1}\PY{p}{:} \PY{k}{True}

\PY{n}{q2}\PY{p}{:} 
\PY{n}{cond2}\PY{p}{:} \PY{p}{(}\PY{n}{v2} \PY{o}{=} \PY{l+m+mi}{10} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n2}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{p}{(}\PY{p}{(}\PY{l+m+mi}{15} \PY{o}{\PYZgt{}} \PY{n}{v0}\PY{p}{)} \PY{o}{\PYZam{}}\PY{o}{\PYZam{}} \PY{o}{!}\PY{n}{n0} \PY{p}{)} 
\PY{n}{cols2}\PY{p}{:} \PY{err}{\PYZob{}}\PY{p}{(}\PY{n}{v4}\PY{p}{,}\PY{n}{n4}\PY{p}{)}\PY{err}{\PYZcb{}}
\PY{n}{Assign2}\PY{p}{:} \PY{k}{True}
\end{Verbatim}


==> conclusion.tex <==
\section{Conclusions}
%
The rise of smart home devices and the Internet of Things 
%has led to the edge becoming major data source for ML inference tasks while providing a new opportunity for low-cost edge-cloud execution.
%
%At the same time, ML inference tasks have grown to consider complex workflows containing multiple inter-connected models (e.g., video analytics), with an ecosystem that provides a variety of model choices through different implementations or transformations (e.g., distillation, compression, quantization).
%
opens up the opportunity  for ML serving systems at the level of both the infrastructure and ML workflow to explore new trade-offs between accuracy and performance.
%
We build {\name}, an ML serving to optimize ML workflows which takes into account the cost, availability, and performance of the increasingly tiered and heterogeneous infrastructures.
%
{\name} significantly reduces the total serving cost of visual question answering and vehicle tracking from the NVIDIA AI City Challenge compared with state-of-the-art solutions.
%

==> shorthand.tex <==
% shorthand: paper-specific shorthand
\newcommand{\apps}[1]{\mathsf{Apps}_{#1}}

\newcommand{\appsof}[1]{\mathsf{Apps}[ #1 ]}

\newcommand{\argsof}[1]{\mathsf{Args}[ #1 ]}

\newcommand{\arityof}[1]{\mathsf{Arity}_{#1}}

\newcommand{\bodies}[1]{\mathsf{Bodies}_{#1}}

\newcommand{\bodyof}[1]{\mathsf{Body}_{#1}}

\newcommand{\calloneref}{\textbf{(5)}\xspace}

\newcommand{\callzeroref}{\textbf{(2)}\xspace}

\newcommand{\chc}[1]{\mathsf{CHC}[ #1 ]}

\newcommand{\chcs}[1]{\mathsf{CHCs}[ #1 ]}

\newcommand{\clauses}[1]{\mathsf{Clauses}[ #1 ]}

\newcommand{\collapse}[2]{\textsc{Collapse}_{#1}^{#2}}

\newcommand{\copyrel}[1]{\textsc{CopyRel}_{#1}}

\newcommand{\corr}[1]{\textsc{Corr}_{#1}}

\newcommand{\ctrof}[1]{\mathsf{Ctr}[#1]}

\newcommand{\ctxrelof}[1]{\mathsf{CtxRel}[ #1 ]}

% array indexing: confirmed
\newcommand{\ctxs}[1]{\mathsf{Ctxs}[ #1 ]}

\newcommand{\dblref}{\textbf{(1)}\xspace}

\newcommand{\degreeof}[1]{\mathsf{deg}(#1)}

\newcommand{\deps}{\textsc{Deps}\xspace}

\newcommand{\depsof}[1]{\mathsf{Deps}_{#1}}

\newcommand{\tdepsof}[1]{\mathsf{TrDeps}_{#1}}

\newcommand{\domainof}[1]{\mathsf{Dom}[ #1 ]}

\newcommand{\duality}{\textsc{Duality}\xspace}

\newcommand{\edgelblof}[1]{\mathsf{EdgeLbl}[ #1 ]}

\newcommand{\eldarica}{\textsc{Eldarica}\xspace}

\newcommand{\elseref}{\textbf{(4)}\xspace}

\newcommand{\expand}[1]{\textsc{Expand}_{#1}}

\newcommand{\expandaux}{\textsc{ExpAux}\xspace}

\newcommand{\expandsto}{\preceq}

\newcommand{\formulas}{\mathsf{Forms}}

\newcommand{\headof}[1]{\mathsf{Head}_{#1}}

\newcommand{\siblingof}[1]{\mathsf{Siblings}_{#1}}

\newcommand{\impact}{\textsc{Impact}\xspace}

\newcommand{\instances}[1]{\mathsf{Instances}[ #1 ]}

\newcommand{\interps}[1]{\mathsf{Interps_{ #1 }}}

\newcommand{\issat}{\textsc{IsSat}\xspace}

\newcommand{\mcchc}{\mathcal{S}_{\cc{MC}}}

\newcommand{\mcpreds}{\mathcal{R}[ \cc{MC} ]}

\newcommand{\mcsolve}{\textsc{SolveCdd}[ \cc{MC} ]}

\newcommand{\nodelblof}[1]{\mathsf{NodeLbl}[ #1 ]}

\newcommand{\nodesof}[1]{\mathsf{Nodes}[ #1 ]}

\newcommand{\nosoln}{\mathsf{None}}

\newcommand{\postctr}[1]{\textsc{Post}_{#1}}

\newcommand{\prectr}[1]{\textsc{Pre}_{#1}}

\newcommand{\predatomsof}[1]{\mathsf{Atoms}_P[ #1 ]}

\newcommand{\predof}[1]{\mathsf{Pred}[ #1 ]}

\newcommand{\queryof}[1]{\mathsf{Query}_{#1}}

\newcommand{\relof}[1]{\mathsf{Rel}[ #1 ]}

\newcommand{\relpreds}{\mathsf{Preds}}

\newcommand{\relsof}[1]{\mathsf{Rels}_{#1}}

\newcommand{\relvarsof}[1]{\mathsf{RelVars}[ #1 ]}

\newcommand{\seahorn}{\textsc{SeaHorn}\xspace}

\newcommand{\shara}[1]{\textsc{Shara}_{#1}}

\newcommand{\sharingclause}{\textsc{SharedRel}\xspace}

\newcommand{\siblings}[1]{\mathsf{Siblings}[ #1 ]}

\newcommand{\singleton}[1]{\textsc{Single}[ #1 ]}

\newcommand{\sinkof}[1]{\mathsf{sink}[ #1 ]}

\newcommand{\solveaux}{\textsc{SAux}\xspace}

\newcommand{\solvecdd}[1]{\textsc{SolveCdd}_{#1}}

\newcommand{\solveitp}{\textsc{Itp}\xspace}

\newcommand{\srcof}[1]{\mathsf{src}[ #1 ]}

\newcommand{\tformulas}[1]{\mathsf{Forms}[ #1 ]}

\newcommand{\thenref}{\textbf{(3)}\xspace}

\newcommand{\unit}{\mathsf{unit}}

\newcommand{\used}[1]{\mathsf{Use}[ #1 ]}

\newcommand{\vars}{\cc{Vars}}

\newcommand{\varsof}[1]{\mathsf{Vars}_{#1}}

%\newcommand{\vc}[1]{\textsc{Cex}_{#1}}

\newcommand{\vinta}{\textsc{Vinta}\xspace}

\newcommand{\vocab}{\mathsf{Vocab}}

\newcommand{\whale}{\textsc{Whale}\xspace}

\newcommand{\zthree}{\textsc{Z3}\xspace}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "p"
%%% End: 


==> sqlcmd.tex <==
%
\newcommand{\sql}{\textsf{q}\xspace}
%
\newcommand{\STable}[1]{\textsf{Scan}(#1)\xspace}
%
\newcommand{\SFilter}[2]{\textsf{Filter}(#1,~#2)\xspace}
%
\newcommand{\SProj}[2]{\textsf{Proj}(#1,~#2)\xspace}
%
\newcommand{\SJoin}[4]{\textsf{Join}(#1,~#2,~#3,~#4)\xspace}
%
\newcommand{\SInnerJoin}[3]{\textsf{Inner Join}(#1,~#2,~#3)\xspace}
%
\newcommand{\SUnion}[2]{\textsf{Union}(#1,~#2)\xspace}
%
\newcommand{\SAggregate}[3]{\textsf{Aggregate}(#1,~#2,~#3)\xspace}
%
\newcommand{\evaluation}[3]{\langle #1 \models #2 \rangle \Downarrow #3\xspace}
%
\newcommand{\MyAlgorithm}{\textsf{MyAlgorithm}\xspace}
%
\newcommand{\construct}{\textsf{construct}\xspace}
%
\newcommand{\train}{\textsf{train}\xspace}
%
\newcommand{\transform}{\textsf{ConstructTran}\xspace}
%
\newcommand{\constructPred}{\textsf{ConstructPred}\xspace}
%
\newcommand{\fresh}{\textsf{Init}\xspace}

%
\newcommand{\expr}{\textsf{e}\xspace}
%
\newcommand{\symexpr}{\textsf{sym-e}\xspace}
%
\newcommand{\column}[1]{\textsf{Column}~#1}
%
\newcommand{\constant}[1]{\textsf{Const}~#1}
%
\newcommand{\bin}[3]{\textsf{Bin}~#1~#2~#3}
%
\newcommand{\binE}[3]{\textsf{BinE}~#1~#2~#3}
%
\newcommand{\binL}[3]{\textsf{BinL}~#1~#2~#3}
%
\newcommand{\Function}[2]{\textsf{Fun}~#1~(#2)}
%
\newcommand{\conexpr}{\textsf{ConstExpr}}
%
\newcommand{\conpred}{\textsf{ConstPred}}
%
\newcommand{\conLogic}{\textsf{ConstLogic}}
%
\newcommand{\conpredAux}{\textsf{ConstPredAux}}
%
\newcommand{\conCom}{\textsf{ConstComp}}
%
\newcommand{\conAnd}{\textsf{ConstAnd}}
%
\newcommand{\conOr}{\textsf{ConstOr}}
%
\newcommand{\pred}{\textsf{p}\xspace}
%
\newcommand{\op}{\textsf{op}}
%
\newcommand{\cp}{\textsf{cp}}
%
\newcommand{\logic}{\textsf{logic}}
%
\newcommand{\buildBin}{\textsf{ConstBin}}
%
\newcommand{\fre}{\textsf{Fresh}}
%
\newcommand{\buildRel}{\textsf{Asg}}
%
\newcommand{\buildNewTuple}{\textsf{NewVec}}
%
\newcommand{\getF}[1]{\textsf{GetFun}~#1}
%
\newcommand{\qconcat}{\textsf{Concat}}
%
%\newcommand{\pred}{\textsf{Pred}}
%
\newcommand{\Not}[1]{\textbf{Not}~#1}
%
\newcommand{\AND}[2]{~#1~\&\&~#2}
%
\newcommand{\OR}[2]{~#1~||~#2}
%
\newcommand{\isNull}[1]{\textbf{IsNull}~#1}
%
\newtheorem{mydef}{Definition}
%
\newtheorem{myeg}{Example}
%
\newtheorem{theorem}{Theorem}


==> std.tex <==
% Standard math shorthand.
\newcommand{\add}[2]{#1 \union \{ #2 \}}

%\newcommand{\assign}{\mathbin{:=}}

\newcommand{\auflia}{\textsc{Auflia}\xspace}

\newcommand{\bigland}{\bigwedge}

\newcommand{\biglor}{\bigvee}

\newcommand{\bigunion}{\bigcup}

\newcommand{\bools}{\mathbb{B}}

\newcommand{\bv}{\textsc{Bv}\xspace}

\newcommand{\code}{\mathtt}

\newcommand{\compose}{\circ}

\newcommand{\concat}{\cdot}

\newcommand{\cons}{\mathbin{::}}

\newcommand{\disjunion}{\dot{\cup}}

\newcommand{\domain}{\mathsf{Dom}}

\newcommand{\elts}[1]{\{ #1 \}}

\newcommand{\entails}{\models}

\newcommand{\euf}{\textsc{Euf}\xspace}

\newcommand{\false}{\mathsf{False}}

\newcommand{\intersection}{\cap}

\newcommand{\ints}{\mathbb{Z}}

\newcommand{\lia}{\textsc{Lia}\xspace}

\newcommand{\nats}{\mathbb{N}}

\newcommand{\none}{\mathsf{None}}

\newcommand{\partto}{\hookrightarrow}

\newcommand{\pset}{\mathcal{P}}

\newcommand{\range}{\mathsf{Rng}}

\newcommand{\remove}[2]{#1 \setminus \{ #2 \}}

\newcommand{\replace}[3]{#1 [ #3 / #2 ]}

\newcommand{\restrict}[2]{#1|_{#2}}

\newcommand{\sats}{\vdash}

\newcommand{\setformer}[2]{\{ #1\ |\ #2 \}}

\newcommand{\some}{\mathsf{Some}}

\newcommand{\subs}[2]{#1 [ #2 ]}

\newcommand{\tc}[1]{#1^{*}}

\newcommand{\true}{\mathsf{True}}

% \newcommand{\undef}{\uparrow}

\newcommand{\union}{\cup}

\newcommand{\upd}[3]{#1[#2 \mapsto #3]}

% Theorem environments
\newtheorem{cor}{\bf{Corollary}}

\newtheorem{defn}{\bf{Definition}}

\newtheorem{ex}{\bf{Example}}

\newtheorem{lem}{\bf{Lemma}}

\newtheorem{thm}{\bf{Theorem}}

% Register classes of stuff to refer to with autoref.
\renewcommand{\algorithmautorefname}{Alg.}

\newcommand{\appautorefname}{App.}

\newcommand{\corautorefname}{Cor.}

\newcommand{\defnautorefname}{Defn.}

\newcommand{\exautorefname}{Ex.}

\newcommand{\figautorefname}{Fig.}

\newcommand{\lemautorefname}{Lemma}

\newcommand{\lineautorefname}{Line}

\newcommand{\thmautorefname}{Thm.}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "p"
%%% End: 



\newcommand{\beibin}[1]{\textcolor{purple}{#1}}


